Representing and Reasoning with Multi-Stakeholder Qualitative Preference Queries

Many decision-making scenarios, e.g., public policy, healthcare, business, and disaster response, require accommodating the preferences of multiple stakeholders. We offer the first formal treatment of reasoning with multi-stakeholder qualitative preferences in a setting where stakeholders express their preferences in a qualitative preference language, e.g., CP-net, CI-net, TCP-net, CP-Theory. We introduce a query language for expressing queries against such preferences over sets of outcomes that satisfy specified criteria, e.g., $\mlangpref{\psi_1}{\psi_2}{A}$ (read loosely as the set of outcomes satisfying $\psi_1$ that are preferred over outcomes satisfying $\psi_2$ by a set of stakeholders $A$). Motivated by practical application scenarios, we introduce and analyze several alternative semantics for such queries, and examine their interrelationships. We provide a provably correct algorithm for answering multi-stakeholder qualitative preference queries using model checking in alternation-free $\mu$-calculus. We present experimental results that demonstrate the feasibility of our approach.

==> appen.tex <==

\setcounter{lemma}{0}
\setcounter{section}{0}
\section*{Appendix}




\section{Implementation Details}
\label{sec:impl}

A prototype implementation is developed in XSB prolog language~\cite{swift2012xsb}. 



\section{Experimental Results}

%\subsection{Case Study}

%\textbf{Todo}


\subsection{Experiments with Random Graphs}




%% single column table.



